Loop Braiding Statistics and Interacting Fermionic Symmetry-Protected Topological Phases in Three Dimensions

We study Abelian braiding statistics of loop excitations in three-dimensional (3D) gauge theories with fermionic particles and the closely related problem of classifying 3D fermionic symmetry-protected topological (FSPT) phases with unitary symmetries. It is known that the two problems are related by turning FSPT phases into gauge theories through gauging the global symmetry of the former. We show that there exist certain types of Abelian loop braiding statistics that are allowed only in the the presence of fermionic particles, which correspond to 3D "intrinsic" FSPT phases, i.e., those that do not stem from bosonic SPT phases. While such intrinsic FSPT phases are ubiquitous in 2D systems and in 3D systems with anti-unitary symmetries, their existence in 3D systems with unitary symmetries was not confirmed previously due to the fact that strong interaction is necessary to realize them. We show that the simplest unitary symmetry to support 3D intrinsic FSPT phases is $\mathbb{Z}_2\times\mathbb{Z}_4$. To establish the results, we first derive a complete set of physical constraints on Abelian loop braiding statistics. Solving the constraints, we obtain all possible Abelian loop braiding statistics in 3D gauge theories, including those that correspond to intrinsic FSPT phases. Then, we construct exactly soluble state-sum models to realize the loop braiding statistics. These state-sum models generalize the well-known Crane-Yetter and Dijkgraaf-Witten models.

==> sec_obstruction.tex <==
\subsection{Obstructions}
To have well-defined topological field theories, we need to make sure that there are no $\mathcal{H}^5$ obstructions. For this purpose we now introduce a series of invariants to distinguish the $\mathcal{H}^5$ cohomology classes.

First of all, given any $5$-cocycle in $\mathcal{Z}^5[G, \mathrm{U}(1)]$, we can form their slant products which are $4$-cocycles. If the $5$-cocycle is cohomologically trivial, so are all the $4$-cocyclces. We can then use the invariants introduced in \Ref{WangLevinPRB} to check whether the $4$-cocycles are cohomologically trivial or not.  Physically, the 2D SET phase obtained from dimensional reduction should be free of gauge anomaly~\cite{Chen2014, BBCW}. In fact, one can generally show that this is indeed the case for Abelian $G$.

The other invariants are more nontrivial. They will be denoted by $\Omega_i, \Omega_{ij}, \Omega_{ijk}$, all modulo $2\pi$. Let us first present the final results:
\begin{equation}
	\begin{split}
		\Omega_i&=\pi\frac{N_0}{N_{0i}}p_{ii}(1+q_i),\\
		\Omega_{ij}&=\pi \frac{N_0}{N_{0j}}\frac{N^{ij}}{N_i}p_{ji}(1+q_i)  + \pi \frac{N_0}{N_{0i}}\frac{N^{ij}}{N_j}(q_ip_{ij}+q_jp_{ii}).\\
	\end{split}
	\label{}
\end{equation}
Notice that $\Omega_{ijk}$ is only sensitive to non-Abelian $3$-cocycles. If any of them is nonzero (mod $2\pi$), or $e^{i\Omega}\neq 1$, the obstruction does not vanish. General expressions of $\Omega_i, \Omega_{ij}$ and $\Omega_{ijk}$ in terms of the $5$-cocycle can be found in.

In the following we write $N_i=2^{r_i}t_i$ for $i=0,1,\dots, K$, where $t_i$'s are odd integers.

\subsubsection{$G=\mathbb{Z}_{N_1}$}
We obtain $\Omega_1=\pi 2^{r_0-\text{min}(r_0,r_1)} p_{11}$.

\begin{enumerate}
	\item If $r_0>r_1$, the obstruction vanishes for any $p_{11}$.
	\item If $r_0\leq r_1$, $\Omega_1=\pi p_1$ and obstruction vanishes for even $p_{11}$.
\end{enumerate}

We also observe that $\Omega_1=N_1\Theta_{1,1}$.

\subsubsection{$G=\mathbb{Z}_{N_1}\times\mathbb Z_{N_2}$}
Without loss of generality we assume $r_1\leq r_2$. We find
\begin{equation}
	\begin{gathered}
	\Omega_{12}=\pi 2^{r_0-\text{min}(r_0,r_1)+r_2-r_1}p_{21},\\
	\Omega_{21}=\pi 2^{r_0-\text{min}(r_0,r_2)}p_{12}.
	\end{gathered}
	\label{}
\end{equation}


